Inaccuracy matters: accounting for solution accuracy in event-triggered nonlinear model predictive control

We consider the effect of using approximate system predictions in event-triggered control schemes. Such approximations may result from using numerical transcription methods for solving continuous-time optimal control problems. Mesh refinement can guarantee upper bounds on the error in the differential equations which model the system dynamics. With the accuracy guarantees of a mesh refinement scheme, we show that the proposed event-triggering scheme -- which compares the measured system with approximate state predictions -- can be used with a guaranteed strictly positive inter-update time. We show that if we have knowledge of the employed transcription scheme or the approximation errors, then we can obtain better online estimates of inter-update times. We additionally detail a method of tightening constraints on the approximate system trajectory used in the nonlinear programming problem to guarantee constraint satisfaction of the continuous-time system. This is the first work to incorporate prediction accuracy in triggering metrics. Using the solution accuracy we can guarantee reliable lower bounds for inter-update times and perform solution dependent constraint tightening.

==> ETC_table.tex <==


% \begin{table*}[t]
% \centering
% \begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c |}
% \hline 
% Paper & Cont. & NL & \cellcolor{gray!50} & \makecell{Output \\ feedback} & Networked &  \cellcolor{gray!50} & \makecell{Threshold \\ inequality} & \makecell{Lyapunov \\ constraint} & \makecell{Time \\ adaptive } & \makecell{Structure \\ based} & \cellcolor{gray!50} & EMPC \\
% \hline \hline
% \cite{eqtami2011novel,li2014event}& \checkmark & \checkmark &\cellcolor{gray!50} &  &  &\cellcolor{gray!50}& \checkmark &  &  &  &\cellcolor{gray!50}&  \\ \hline 
% \cite{eqtami2011event}&  & \checkmark &\cellcolor{gray!50} &  &  &\cellcolor{gray!50}& \checkmark &  &  &  &\cellcolor{gray!50}&  \\ \hline 
% %\cite{li2014event}& \checkmark & \checkmark &\cellcolor{gray!50} &  &  &\cellcolor{gray!50}& \checkmark &  &  &  &\cellcolor{gray!50}&  \\ \hline 
% \cite{yao2013networked,yao2013resource}& \checkmark & \checkmark &\cellcolor{gray!50} &  & \checkmark &\cellcolor{gray!50}& \checkmark & \checkmark &  &  &\cellcolor{gray!50}&  \\ \hline 
% \cite{zhang2013lyapunov}& \checkmark & \checkmark &\cellcolor{gray!50} & \checkmark &  &\cellcolor{gray!50}& \checkmark & \checkmark &  &  &\cellcolor{gray!50}& \\ \hline 
% \cite{zhang2014economic}& \checkmark & \checkmark &\cellcolor{gray!50} & \checkmark &  &\cellcolor{gray!50}& \checkmark & \checkmark &  &  &\cellcolor{gray!50}& \checkmark \\ \hline 
% \cite{he2015event}& \checkmark & \checkmark &\cellcolor{gray!50} &  &  &\cellcolor{gray!50}& \checkmark & \checkmark &  &  &\cellcolor{gray!50}&  \\ \hline 
% \cite{lehmann2013event}&  &  &\cellcolor{gray!50} &  &  &\cellcolor{gray!50}& \checkmark &  &  &  &\cellcolor{gray!50}&  \\ \hline 
% \cite{hashimoto2015time,hashimoto2017event}& \checkmark & \checkmark &\cellcolor{gray!50} &  &  &\cellcolor{gray!50}&\checkmark  &  & \checkmark &  &\cellcolor{gray!50}&  \\ \hline 
% \cite{jost2015optimal,darup2017novel,berner2016comparison}&  &  &\cellcolor{gray!50} &  &  &\cellcolor{gray!50}&  &  &  & \checkmark &\cellcolor{gray!50}&  \\ \hline 
% \cite{bernardini2012energy}&  &  &\cellcolor{gray!50} & \checkmark & \checkmark &\cellcolor{gray!50}&  &  &  & \checkmark &\cellcolor{gray!50}&  \\ \hline 
% \end{tabular} 
% \caption{Comparison of ET-MPC related publications}
% \label{tab:label}
% \end{table*}



==> oldProofs.tex <==

% \begin{proof}
%     The ETC, \eqref{eq:EventTriggeringCondition} guarantees that
%     \begin{equation}
%         \norm{\tilde{x}_1(t) - y_1(t)} + \hdots + \norm{\tilde{x}_n(t) - y_n(t)} \leq \Delta.
%     \end{equation}
%     For succinctness we write $f(t,x,u)$ as $f(x)$. Without loss of generality, assume problem \eqref{eq:Bolza_cont} was last solved at time $t_i^u=0$, parameterized by the measurement $\tilde{x}(0)=y(0)$. Then the prediction error in the $i^\text{th}$ state is
%     \begin{align} \label{eq:th1_1}
%         \delta_i(t) &= \int_0^t \dot{\tilde{x}}_i(\tau) - \dot{y}_i(\tau) \mathrm{d}\tau \\
%         &= \int_0^t \dot{\tilde{x}}_i(\tau) - \left(f_i(x(\tau)) + v_i(\tau) +  \dot{\theta}_i(\tau)\right) \mathrm{d}\tau \\
%         &= \underbrace{\int_0^t \dot{\tilde{x}}_i(\tau) - \left(f_i(x(\tau)) + v_i(\tau)\right) \mathrm{d}\tau}_{:=\gamma_i(t)} + \theta_i(t)-\theta_i(0)
%     \end{align}
%     Having isolated the measurement noise, we focus on the integral denoted by $\gamma_i(t)$. By noting that scalar $w_i$ is strictly positive and not a function of time, we may rewrite \eqref{eq:RLE} as
%     \begin{equation}
%         \epsilon_{k,i} = \int_{t_k}^{t_{k+1}}\underbrace{\norm{\frac{\dot{\tilde{x}}_i(\tau) - f_i(\tilde{x}(\tau))}{w_i+1}}}_{:=\norm{\alpha_i(\tau)}}\mathrm{d}\tau.
%     \end{equation}
%     Subsequent substitution of $\dot{\tilde{x}}(t)= (w_i+1)\alpha(t) + f_i(x(t))$ into \eqref{eq:th1_1} results in
%     \begin{equation}
%         \gamma_i(t) = \int_0^t (w_i+1)\alpha_i(\tau) + f_i(\tilde{x}(\tau))-f_i(x(\tau)) - v_i(\tau)\mathrm{d}\tau
%     \end{equation}
%     Through application of the triangle inequality, the prediction error magnitude of each state may be bounded from above as
%     \begin{align}
%         \norm{\gamma_i(t)} &\leq \norm{(w_i+1)\int_0^t\alpha_i(\tau)\mathrm{d}\tau} \notag \\
%         & + \norm{\int_0^t f_i(\tilde{x}(\tau))-f_i(x(\tau))\mathrm{d}\tau} + \norm{\int_0^t -v_i(\tau)\mathrm{d}\tau} \\
%         &\leq (w_i+1)\int_0^t\norm{\alpha_i(\tau)}\mathrm{d}\tau \notag \\
%         & + \int_0^t \norm{f_i(\tilde{x}(\tau))-f_i(x(\tau))} \mathrm{d}\tau + \int_0^t \norm{v_i(\tau)}\mathrm{d}\tau \label{eq:ThreeIntegrals_1}.
%     \end{align}
%     Now, consider the set $\mathcal{T}_{t} \subseteq \mathcal{T}_h$ of open intervals of $T$, i.e.
%     \begin{equation}
%         \mathcal{T}_{t} := \{T \in \mathcal{T}_h | T \cap \overline{(0,t)} \not = \emptyset\}
%     \end{equation}
%     which is a mesh on $\Omega_t := (0,t)$ and by construction satisfies the properties detailed in Definition~\ref{def:Mesh}. Since the mesh refinement scheme guarantees $\epsilon_{k,i} \leq \hat{\epsilon}_i, \forall i \in \{1,\hdots,n\}$, the first term in \eqref{eq:ThreeIntegrals_1} may be bounded from above as,
%     \begin{align}
%         (w_i + 1)\int_0^t\norm{\alpha_i(\tau)}\mathrm{d}\tau &\leq (w_i + 1)\sum_{T \in \mathcal{T}_{t}} \int_T \norm{\alpha_i(\tau)}\mathrm{d}\tau  \\
%         &\leq (w_i+1) \sum_{T \in \mathcal{T}_{t}} \hat{\epsilon}.
%     \end{align}
%     Through application of the resolution and quasi-uniformity properties of mesh $\mathcal{T}_t$, the smallest interval satisfies
%     \begin{equation}
%     \min_{T\in\mathcal{T}_t} \norm{T} \geq \sigma h := \underline{h}.
%     \end{equation}
%     Using $\ceil{\cdot}$ to denote the ceiling function, we may bound the maximum number of mesh segments in the interval $(0,t)$ as $\ceil{t\underline{h}^{-1}}$, from which it follows that,
%     \begin{equation}
%         \sum_{T \in \mathcal{T}_{t}} \hat{\epsilon}_i \leq \ceil*{\frac{t}{\underline{h}}} \hat{\epsilon}_i \leq \left(\frac{t}{\underline{h}}+1\right) \hat{\epsilon}_i.
%     \end{equation}
%     From this, and by noting that $\vecnorm{\theta(t)-\theta(0)} \leq 2\hat{\theta}$ by assumption, we may bound the prediction error magnitude as,
%     \begin{equation}\label{eq:ThreeIntegrals_2}
%         \begin{split}
%         \vecnorm{\delta(t)} & \leq \left(\frac{t}{\underline{h}}+1\right)  (w+1)^\intercal\hat{\epsilon} + 2\hat{\theta}\\
%         & + \int_0^t \vecnorm{f(\tilde{x}(\tau)) - f(x(\tau))}\mathrm{d}\tau + \int_0^t\vecnorm{-v(\tau)}\mathrm   {d}\tau.
%         \end{split}
%     \end{equation}
%     From the assumption of Lipschitz continuity of $f(\cdot)$ the first integral in \eqref{eq:ThreeIntegrals_2} is bounded by
%     \begin{equation}
%         \int_0^t \vecnorm{f(\tilde{x}(\tau)) - f(x(\tau))}\mathrm{d}\tau \leq  \int_0^t L_x\vecnorm{\delta(\tau)}\mathrm{d}\tau \leq tL_x\Delta.
%     \end{equation}
%     By assumption, the second integrand in \eqref{eq:ThreeIntegrals_2} satisfies $\vecnorm{v(t)} \leq \hat{v}$. Therefore, since $\vecnorm{w} \leq \hat{w}$ and $w_i\geq 0,\ \forall i \in \{1,\hdots,n\}$,
%     \begin{equation} \label{eq:PreErrorNorm1}
%         \vecnorm{\delta(t)} \leq \left(\frac{t}{\underline{h}}+1\right)  (\hat{w}+1)^\intercal\hat{\epsilon} + t\left(L_x \Delta + \hat{v}\right) + 2\hat{\theta}.
%     \end{equation}
%     We may guarantee the existence of $\underline{\tau}^u > 0$ by showing the existence of a $t>0$ such that
%     \begin{equation}
%         \left(\frac{t}{\underline{h}}+1\right) (\hat{w}+1)^\intercal\hat{\epsilon} + t\left(L_x \Delta + \hat{v}\right) + 2\hat{\theta} \leq \Delta.
%     \end{equation}
%     Through manipulation, this inequality is satisfied when
%     \begin{equation}
%         t \leq \frac{\Delta - (\hat{w}+1)^\intercal\hat{\epsilon} - 2\hat{\theta}}{\frac{(\hat{w}+1)^\intercal\hat{\epsilon}}{\sigma h} + L_x\Delta + \hat{v}}.
%     \end{equation}
%     Since all parameters are in $\mathbb{R}_0^+$, the RHS is guaranteed to be strictly positive as long as $\Delta > (\hat{w}+1)^\intercal\hat{\epsilon} + 2\hat{\theta}$.
% \end{proof}


% \section{Online estimation of IUT} \label{sec:OnlineTrig}
% The IUT bound \eqref{eq:min_IUT} can be imrpoved by using the actual error information provided by solving \eqref{eq:Bolza_cont} with a mesh refinement procedure. 
% This is the first explicit definition of IUT to account for both problem data and the solution accuracy of \eqref{eq:Bolza_cont}.
% Although the following results resemble STC conditions of the form \eqref{eq:STC_Prob_Condition}, we make no claims about stability or performance of control based on these conditions.
% Additional assumptions on problem structure would be needed for this.
% Instead, we simply provide estimates of IUTs, which may be useful for process/resource scheduling. 
  
% First, we determine a lower bound on $\tau_i^u$, not dependent on~$\eta_k$, through using knowledge of the collocation constraints. This may be applicable in the case

% \begin{theorem}[Collocation Triggering (CT)]
% 	Let $L_{p,k}$ be the Lipschitz constant of the approximating polynomial used in segment $T_k$. The IUT
% 	\begin{equation} \label{eq:trig_CT}
% 	\begin{split}
% 	& \tau_i^\text{CT} = \sup \Bigg\{\tau \in \mathbb{R}^+ |   t(L_x \Delta + \hat{v}) + \\
% 	& 2\hat{\theta} + \vecnorm{(\hat{w}+1)}\Bigg(\sum_{k\in\mathcal{K}_t}\int_{T_k} n L_{p,k} \norm{\tau-t_k^\text{col}} + \\
%      & L_x\vecnorm{\tilde{x}(t_k^\text{col})- \tilde{x}(\tau)}\mathrm{d}\tau\Bigg) \leq \Delta \Bigg\}
% 	\end{split}
% 	\end{equation}
% 	calculated from the approximate solution $\tilde{x}(\cdot)$ to problem~\eqref{eq:Bolza_cont} at time $t_i^u$ satisfies $\vecnorm{\delta(t_i^u+\tau)} \leq \Delta, \forall \tau \leq \tau_i^\text{CT}$.
% \end{theorem}
% \begin{proof}
% 	We begin by noting that
% 	\begin{equation} \label{eq:CT1}
% 	\int_0^t \norm{\dot{\tilde{x}}_i(\tau) - f_i(\tilde{x}(\tau))} \mathrm{d}\tau \leq \sum_{k\in\mathcal{K}_t}\int_{T_k}\norm{\dot{\tilde{x}}_i(t) - f_i(\tilde{x}(\tau))} \mathrm{d}\tau,
% 	\end{equation}
% 	where the inequality follows from $\sup{T_k} \geq t$. As \eqref{eq:dynODE} are satisfied exactly at points $t_k^\text{col}$, we may write \eqref{eq:CT1} as,
% 	\begin{align}
% 	&\sum_{k\in\mathcal{K}_t}\int_{T_k} \norm{\dot{\tilde{x}}_i(\tau) - \dot{\tilde{x}}_i(t_k^\text{col}) + f_i(\tilde{x}(t_k^\text{col}))- f_i(\tilde{x}(\tau))}\mathrm{d}\tau \\
% 	&\leq \sum_{k\in\mathcal{K}_t}\int_{T_k} \norm{\dot{\tilde{x}}_i(\tau) - \dot{\tilde{x}}_i(t_k^\text{col})} + \norm{f_i(\tilde{x}(t_k^\text{col}))- f_i(\tilde{x}(\tau))}\mathrm{d}\tau.
% 	\end{align}
% 	Summing this error expression for each  state results in,
% 	\begin{align}
% 	&\int_0^t\vecnorm{\varepsilon(\tau)}\mathrm{d}\tau   \\
% 	& \leq \sum_{k\in\mathcal{K}_t}\int_{T_k} \vecnorm{\dot{\tilde{x}}(\tau) - \dot{\tilde{x}}(t_k^\text{col})} + \vecnorm{f(\tilde{x}(t_k^\text{col}))- f(\tilde{x}(\tau))}\mathrm{d}\tau \\
% 	& \leq \sum_{k\in\mathcal{K}_t}\int_{T_k} n L_{p,k} \norm{\tau-t_k^\text{col}} + L_x\vecnorm{\tilde{x}(t_k^\text{col})- \tilde{x}(\tau)}\mathrm{d}\tau.
% 	\end{align}
% 	where the second inequality results from noting that all polynomials $\in \mathcal{P}_p(T_k)$ defined on bounded set $T_k$ are Lipschitz functions, and using $L_{p,k}$ to denote the Lipschitz constant of the approximating polynomial used in segment~$T_k$.
% 	Substituting this quadrature error bound into \eqref{eq:PreErrorNorm1} in place of $(t\underline{h}^{-1}+1)\hat{\epsilon}$ results in
% 	\begin{equation}
% 	\begin{split}
%     \vecnorm{\delta(t)} \leq  t(L_x \Delta & + \hat{v}) + 2\hat{\theta} +\\ \vecnorm{(\hat{w}+1)}&\Bigg(\sum_{k\in\mathcal{K}_t}\int_{T_k} n L_{p,k} \norm{\tau-t_k^\text{col}} + \\
%      & L_x\vecnorm{\tilde{x}(t_k^\text{col})- \tilde{x}(\tau)}\mathrm{d}\tau\Bigg).
%      \end{split}
%      \end{equation}
% 	Restricting the RHS to be $ \leq \hat{\epsilon}$ yields the explicitly defined IUT given in \eqref{eq:trig_CT}.
% 	\hspace*{\fill} \qed
% \end{proof}

% For low-order $h$ methods in particular, $L_{p,k}$ may be easily evaluated for each segment $T_k$. 

% \begin{theorem}[Quadrature Error Triggering (QET)]\label{th:QET}
%     The IUT
%     \begin{equation}\label{eq:trig_QET}
%         \begin{split}
%             \tau_i^\text{QET} = \sup  \Bigg\{\tau >0  | \vecnorm{\delta(t)}  \leq \Bigg(\sum_{i=1}^n  \Big((w_i & +1)\sum_{k\in\mathcal{K}_t} \epsilon_{k,i}\Big) + \\ & 2\hat{\theta} + \hat{v}\tau\Bigg) e^{L_x \tau} \leq \Delta  \Bigg\}
%         \end{split}
% \end{equation}
% 	determined from $\tilde{x}(\cdot)$, $\eta_k$, which approximately solves problem \eqref{eq:Bolza_cont} at time $t_i^u$, satisfies $\vecnorm{\delta(t_i^u+\tau)} \leq \Delta, \forall \tau \leq \tau_i^\text{QET}$. Furthermore, $\tau_i^\text{QET} \geq \underline{\tau}^u$.
% \end{theorem}
% \begin{proof}
%     Employing the notation introduced in the proof of Theorem~\ref{th:MinIUTRel}, we begin by noting that
%     \begin{equation}
%         (w_i+1) \int_0^t\norm{\alpha_i(\tau)}\mathrm{d}\tau \leq (w_i+1)\sum_{k \in \mathcal{K}_t} \epsilon_{k,i},
%     \end{equation}
% 	where the inequality follows from $\sup \norm{\mathcal{T}_t} \geq t$. Substituting this into \eqref{eq:ThreeIntegrals_2} and evaluating the second integral, we may bound the prediction error norm at $t\in[t_i^u,t_{i+1}^u)$,
% 	\begin{equation}
% 	\begin{split}
%         \vecnorm{\delta(t)}  \leq \sum_{i=1}^n & \left((w_i+1)\sum_{k\in\mathcal{K}_t} \epsilon_{k,i}\right) + 2\hat{\theta} + \hat{v}t\\
%         & + \int_0^t \vecnorm{f(\tilde{x}(\tau)) - f(x(\tau))}\mathrm{d}\tau.
%         \end{split}
% 	\end{equation}
% 	From the assumption on Lipshitz continuity of $f(\cdot)$,
% 	\begin{equation}
% 	\begin{split}
%         \vecnorm{\delta(t)}  \leq \sum_{i=1}^n & \left((w_i+1)\sum_{k\in\mathcal{K}_t} \epsilon_{k,i}\right) + 2\hat{\theta} + \hat{v}t\\
%         & + \int_0^t L_x\vecnorm{\delta(\tau)}\mathrm{d}\tau.
%         \end{split}
% 	\end{equation}
% 	Instead of bounding the integral with the ETC variable $\Delta$, we employ the Gronwall-Bellman inequality, resulting in
% 	\begin{equation} \label{eq:PreErrorNorm2}
%         \vecnorm{\delta(t)}  \leq \Bigg(\sum_{i=1}^n \left((w_i+1)\sum_{k\in\mathcal{K}_t} \epsilon_{k,i}\right) + 2\hat{\theta} + \hat{v}t\Bigg) e^{L_x t}.
% 	\end{equation}
%     Restricting the RHS to be $ \leq \Delta$ results in the explicitly defined IUT given in \eqref{eq:trig_QET}. As
%     \begin{equation}
%         \sum_{i=1}^n (w_i+1)\sum_{k \in \mathcal{K}_t} \epsilon_{k,i} \leq  \left(\frac{t}{\underline{h}}+1\right),
%     \end{equation}
%     we guarantee that $\tau^\text{QET}_i \geq \underline{\tau}^u$.
% \end{proof}

% Another advantage of the online calculation is that it does not require explicit knowledge of bounds on $w$. 
% In the same fashion as Corollary~\ref{cor:absoluteMinIUT}, we may determine a similar triggering estimate if considering refinement on the absolute local error of each state.

% The mesh refinement procedure may not return the approximation error over arbitrary intervals. Software such as \texttt{ICLOCS2} \cite{nie2018iclocs2} returns $\eta_k$ corresponding to $T_k$. Depending on how the integral is evaluated we may not know the distribution of $\varepsilon(t)$ over this interval. 

% \begin{remark}
%     To this point the analysis has made no assumptions on problem structure. As such it is equally applicable to the different classes of ET-MPC formulations outlined in Section~\ref{sec:preliminaries}.
% \end{remark}

% \section{Constraint tightening} \label{sec:constraintTightening}

% The proposed triggering conditions do not account for state proximity to constraint bounds. We wish to guarantee satisfaction of constraints \eqref{eq:pathConstriants} for the entire prediction horizon $t \in [t_0, t_f]$. 
% However, when solving the transcribed NLP corresponding to problem \eqref{eq:Bolza_cont}, the constraints $c(\tilde{x}(t),u(t),t) \leq 0$ are only enforced on the approximate trajectory $\tilde{x}(\cdot)$ at a finite number of time instances: the mesh points $\mathcal{T}_m$. 
% One way to guarantee that the actual state $x(\cdot)$ complies with state constraints is to employ constraint tightening methods. 
% For the following analysis we only consider the case where $c(\tilde{x}(t),u(t),t) \leq 0$ can be written as the inclusion,
% \begin{equation}
%     \tilde{x}(t) \in \mathbb{X}, \forall t \in [t_0,t_f],
% \end{equation}
% where the constraint set $\mathbb{X}$ satisfies the following assumption.
% \begin{assumption}\label{ass:Nonempty}
% The set $\mathbb{X}$ is closed and convex, and the reduced set,
% \begin{equation}
%     \mathbb{X} \ominus \left\{x \in \mathbb{R}^n \mid x \leq \Delta \right\},
% \end{equation}
% where $\ominus$ denotes the Pontryagon difference, is non-empty.
% \end{assumption}

% Where in the above assumption we have defined the Pontryagon difference of two sets $\mathcal{A}$ and $\mathcal{B}$ is defined as $\mathcal{A} \ominus \mathcal{B} := \{a \in \mathbb{R}^n | a+b \in \mathcal{A}, \forall b \in \mathcal{B}\}$.
% Similarly, we define the Minkowski sum $\oplus$ of $\mathcal{A}$ and $\mathcal{B}$ as $\mathcal{A} \oplus \mathcal{B} := \{a + b | a \in \mathcal{A}, b \in \mathcal{B}\}$. We would not expect this assumption to be particularly restrictive as $\Delta$ will be quite small in practice.
% In the following lemma we evaluate how much state constraints on the approximate solution $\tilde{x}$ must be tightened in order to guarantee that the actual state $x \in \mathbb{X}$.

% \begin{lemma}\label{lemma:ConstraintTightening}
%     Consider a mesh refinement scheme using the relative local error \eqref{eq:RelLocErrBound} or absolute local error \eqref{eq:AbsoluteQuadrature} as a termination criteria.
%     If the approximate trajectory at time $t_k^u+s, s \geq 0,$ predicted from measurement at time $t_k^u$ satisfies $\tilde{x}(t_k^u,s) \in \mathbb{X}_{s},$ where
%     \begin{equation} \label{eq:infTightening}
%         \mathbb{X}_{s} := \mathbb{X} \ominus \mathcal{B}_{s},
%     \end{equation}
%     and the ball $\mathcal{B}_s$ is defined as
%     \begin{equation}
%         \mathcal{B}_{s} := \Bigg\{x \in \mathbb{R}^n \mid 
%       \vecnorm{x} \leq \min\Big\{  \left(\sum_{T \in \mathcal{T}_{s}}\hat{\xi} + 2\hat{\theta} + \hat{v}s\right) e^{L_x s}, \Delta \Big\}\Bigg\},
%     \end{equation}
%     where $\hat{\xi}:=\left(\hat{w}+1\right)^\intercal\hat{\epsilon}$ or $\hat{\xi}:=\hat{\epsilon}$ depending on the refinement termination criteria, then the actual state trajectory satisfies $x(s) \in \mathbb{X}$.
% \end{lemma}

% \begin{proof}
%     From the inequality \eqref{eq:PreErrorNorm2} used in the proof of Theorem~\ref{th:QET} we directly bound the norm between the approximate predicted and measured state at time $t_k^u+s$,
%     \begin{equation}
%         \vecnorm{\delta(t_k^u+s)} \leq \left(\sum_{, \in \mathcal{K}_s} (\hat{w}+1))^\intercal\hat{\epsilon} + 2\hat{\theta} + \hat{v}t\right)e^{L_xt}.
%     \end{equation}
%     Since the ETC scheme guarantees that the control and associated prediction is updated if $\vecnorm{\delta(s)} \geq \Delta$, we can make the bound less conservative as 
%     \begin{equation}
%         \vecnorm{\delta(t_k^u+s)} \leq \min\left\{\left(\sum_{k \in \mathcal{K}_s} (\hat{w}+1))^\intercal\hat{\epsilon} + 2\hat{\theta} + \hat{v}t\right)e^{L_xt}, \Delta\right\}.
%     \end{equation}
%     Tightening the constraint set $\mathbb{X}$ by the RHS of this inequality results in $\mathbb{X}_s$ and guarantees that the actual trajectory $x(t) \in \mathbb{X}, \forall t \in [t_k^u,t_{k+1}^u]$.
%     By Assumption~\ref{ass:Nonempty}, $\mathbb{X}_{s}$ is nonempty $\forall s \in [t_k^u,t_k^u+T_\text{op})$.
% \end{proof}

% Lemma~\ref{lemma:ConstraintTightening} shows that the amount of constraint tightening required depends on the solution accuracy, allowed prediction error $\Delta$, as well as measurement and disturbance noise bounds. This tightening is shown in Figure~\ref{fig:ConstraintTighteningExample}. 
% However the constraint $\tilde{x}(t) \in \mathbb{X}_s$ would still need to be applied at the infinite number of time instances $[t_k^u,t_k^u + T_\text{op}]$. 
% We now adapt \cite[Theorem 1]{fontes2018guaranteed} to show how further tightening of the constraint sets $\mathbb{X}_{s}$ at the mesh points $\mathcal{T}_m$ can be used to guarantee constraint satisfaction of the continuous time OCP.

% Similar to the method proposed in \cite{fontes2018guaranteed}, we define the signed distance frunction from a point $x\in\mathbb{R}^n$ to the set $\mathcal{A}$ as
% \begin{equation}
%     d_{\mathcal{A}}(x) := \min_{y\in\mathcal{A}}\vecnorm{x-y} - \inf_{z\in \mathcal{A}^C}\vecnorm{x-z},
% \end{equation}
% where $\mathcal{A}^C$ denotes the complement of $\mathcal{A}$.
% With this distance function we may rewrite the tightened state constraints from Lemma~\ref{lemma:ConstraintTightening} as
% \begin{equation}
%     d_{\mathbb{X}_s}(\tilde{x}(t_k^u,s)) \leq 0, \forall s \in [t_k^u,t_k^u + T_\text{op}].
% \end{equation}
% The next step is to tighten the constraints on the approximate system at the finite set of mesh points $\mathcal{T}_m$, in order to guarantee constraint satisfaction of the real system over the entire time horizon. This is formalized in the following theorem.

% \begin{theorem} \label{th:tight}
%     Consider a mesh refinement scheme using the relative local error \eqref{eq:RelLocErrBound} or absolute local error \eqref{eq:AbsoluteQuadrature} as a termination criteria. If we define
%     \begin{equation}
%         \alpha_k \geq (\hat{w}+1)^\intercal\hat{\epsilon} + L_f\norm{T_k} + g(t_k^m,t_{k+1}^m), \forall k \in \mathcal{K}_h,
%     \end{equation}
%     and the predicted trajectory $\tilde{x}(\cdot)$ satisfies
%     \begin{equation}
%         d_{\mathbb{X}_{t_k^m}}(\tilde{x}(t_k^m)) \leq -\alpha_k, \forall k \in \mathcal{K}_h,
%     \end{equation}
%     then
%     \begin{equation}
%      d_{\mathbb{X}_{s}}(\tilde{x}(s)) \leq 0, \forall s \in [t_k^m,t_{k+1}^m], k \in \mathcal{K}_h,
%     \end{equation}
%     and further, 
%     \begin{equation}
%         x(t) \in \mathbb{X}, \forall s \in [t_i^u, t_{i+1}^u]
%     \end{equation}
% \end{theorem}
% \begin{proof}
%     From the definition of the tightened constraint set $\mathbb{X}_{s}$ in Lemma~\ref{lemma:ConstraintTightening},
%     \begin{equation}
%         \mathbb{X}_{s} \subseteq \mathbb{X}_{t_k^m}, \forall s \in (t_k^m,t_{k+1}^m].
%     \end{equation}
%     We use the notation $\partial \mathcal{A}$ to denote the boundary of the set $\mathcal{A}$. 
%     Since $\mathbb{X}$ is convex by Assumption~\ref{ass:Nonempty}, the sets $\mathbb{X}_s$ will be convex by construction. Therefore the shortest distance from any point in $\partial\mathbb{X}_s$ to $\partial \mathbb{X}_{t_k^m}$ is equal, satisfying
%     \begin{equation}
%         \min_{y_1 \in \partial \mathbb{X}_{s}} \vecnorm{x_1-y_1} = 
%         \min_{y_2 \in \partial \mathbb{X}_{s}} \vecnorm{x_2-y_2}, \forall x_1,x_2 \in \partial \mathbb{X}_{t_k^m}.
%     \end{equation}
%     From the definition of the sets $\mathbb{X}_s$ in \eqref{eq:infTightening} we define this distance $g : \mathbb{R}^+ \times \mathbb{R}^+ \rightarrow \mathbb{R}^+$ between $\mathbb{X}_S$ and $\mathbb{X}_{t_k^m}$ as
%     \begin{equation}
%         g(s,t_k^m) := 
%         \min \big\{(\beta + \hat{v}s)e^{L_x s},\Delta  \big\} - \min \big\{(\beta + \hat{v}t_k^m)e^{L_x t_k^m},\Delta \big\},
%     \end{equation}
%     where,
%     \begin{equation}
%         \beta := \sum_{T \in  \mathcal{T}_{k+1}^m} \hat{\xi} + 2\sigma.
%     \end{equation}
%     From Assumption~\ref{ass:Nonempty} on the non-emptiness of $\mathbb{X}_s$, $g(\cdot)$ is always well defined.
%     We now consider the approximate state trajectory $\tilde{x}(\cdot)$ at times $t_k^m$ and $s\geq t_k^m$. 
%     Then,
%     \begin{align}
%         \norm{d_{\mathbb{X}_{s}}(\tilde{x}(s)) - d_{\mathbb{X}_{t_k^m}}(\tilde{x}(t_k^m))} &\leq \vecnorm{\tilde{x}(s)-\tilde{x}(t_k^m)} + g(s,t_k^m) \\ 
%         &= \vecnorm{\int_{t_k^m}^s\dot{\tilde{x}}(t)\mathrm{d}t} + g(s,t_k^m) \\
%         & \leq \int_{t_k^m}^{s} \vecnorm{\dot{\tilde{x}}(t)} \mathrm{d}t + g(s,t_k^m).
%     \end{align}
%     Application of the triangle inequality to the mesh refinement conditions \eqref{eq:RelLocErrBound} yields 
%     \begin{align}
%         \int_{T_k} \vecnorm{\dot{\tilde{x}}(t)}\mathrm{d}t - 
%         \int_{T_k} \vecnorm{f(\tilde{x}(t))}\mathrm{d}t &\leq 
%         \int_{T_k} \vecnorm{\dot{\tilde{x}}(t)-f(\tilde{x}(t))}\mathrm{d}t \\ & \leq (\hat{w}+1)^\intercal\hat{\epsilon},
%     \end{align}
%     from which,
%     \begin{align}
%          \int_{t_k^m}^s \vecnorm{\dot{\tilde{x}}(t)}\mathrm{d}t \leq \int_{T_k} \vecnorm{\dot{\tilde{x}}(t)}\mathrm{d}t &\leq \hat{\xi} + \int_{T_k} \vecnorm{f(\tilde{x}(t))}\mathrm{d}t \\
%         & \leq \hat{\xi} + L_f\norm{T_k}.
%     \end{align}
%     Therefore we may bound the distance as
%     \begin{equation}
%         d_{\mathbb{X}_{s}}(\tilde{x}(s)) - d_{\mathbb{X}_{t_k^m}}(\tilde{x}(t_k^m)) \leq \hat{\xi} + L_f\norm{T_k} + g(s,t_k^m).
%     \end{equation}
    
%     We now need to prove that there is no $s < t_{k+1}^m$ for which $d_{\mathbb{X}_{s}}(\tilde{x}(s)) = 0$. Following the argument in \cite{fontes2018guaranteed}, assume $\exists s_1 < t_{k+1}^m$ such that 
%     \begin{equation}
%         d_{\mathbb{X}_{s_1}}(\tilde{x}(s_1)) = 0 \text{ and } d_{\mathbb{X}_{s}}(\tilde{x}(s)) > 0, \forall s \in (s_1,t_{k+1}^m].
%     \end{equation}
%     Therefore, 
%     \begin{align}
%         d_{\mathbb{X}_{s_1}}(\tilde{x}(s_1)) &\leq d_{\mathbb{X}_{t_k^m}}(\tilde{x}(t_k^m)) +  \hat{\xi} + L_f(s_1-t_k^m) + g(s_1,t_k^m) \\ 
%         &\leq -\alpha_k +  \hat{\xi} + L_f(s_1-t_k^m) + g(s_1,t_k^m)) \\
%         & < -\alpha_k + \hat{\xi} + L_f\norm{T_k} + g(t_k^m,t_{k+1}^m) \leq 0.
%     \end{align}
%     which contradicts our assumption. Therefore we may conclude that
%     \begin{equation}
%         d_{\mathbb{X}_s}(\tilde{x}(s)) \leq 0, \forall s \in [t_k^m, t_{k+1}^m], \forall k \in \mathcal{K}_h.
%     \end{equation}
%     Combining this with the results of Lemma~\ref{lemma:ConstraintTightening} guarantees
%     \begin{equation}
%         d_\mathbb{X}(x(t)) \leq 0, \forall t \in [t_i^u,t_{i+1}^u].
%     \end{equation}
% \end{proof}

% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Images/ConstraintTighteningExample_PPT}
% 	\caption[TODO]{A pictorial representation of the proposed constraint tightening method for the constraint set $\mathbb{X}:= [\underline{x},\overline{x}]$. $\mathbb{X}$ is tightened to the set $\mathbb{X}_s$ due to the difference between approximate and actual trajectories. The constraints enforced at discrete mesh points are further tightened depending on the length of the succeeding segment, shown by the green crosses.}
% 	\label{fig:ConstraintTighteningExample}
% \end{figure}

% Theorem~\ref{th:tight} shows that the constraints enforced at each mesh point $t_k^m$ should be tightened by an amount affine in the length of the succeeding mesh segment $\norm{T_k}$ and dependent on the metric of allowable ODE errror $\hat{\xi}$.
% This guarantees that the approximate trajectory is admissible for all time. The constraints must be further tightened by an amount $g(\cdot)$ which relates the difference between approximate and actual trajectories.

% We could use this result to propose an OCP solution scheme where the constraints are tightened at each iteration of the refinement process in accordance with the results in Theorem~\ref{th:tight}. As the mesh becomes increasingly refined, the constraints will become more and more relaxed. In this way constraint satisfaction of the true state $x(t)$ would be guaranteed at every iteration of the refinement procedure. However, we find in practice that this procedure is particularly conservative, especially for very coarse meshes, and may effect the feasibility of the problem. This is particularly important for the initial solves. We could instead start with a finer mesh, but this has adverse effects on solution time. 

% Instead we consider a two part procedure detailed in Algorithm~\ref{alg:MR}. From the condition in Theorem~\ref{th:tight},
% \begin{equation}
%      \norm{d_{\mathbb{X}_{s}}(\tilde{x}(s)) - d_{\mathbb{X}_{t_k^m}}(\tilde{x}(t_k^m))} \leq \vecnorm{\tilde{x}(s)-\tilde{x}(t_k^m)} + g(s,t_k^m),
% \end{equation}
% we can guarantee that $d_{\mathbb{X}_{t_{k+1}^m}}(\tilde{x}(t_{k+1}^m)) \leq 0$ if
% \begin{equation} \label{eq:tight_iter}
%     d_{\mathbb{X}_{t_{k}^m}}(\tilde{x}(t_{k}^m)) \leq \underbrace{\max_{s \in T_k} \vecnorm{\tilde{x}(s) - \tilde{x}(t_k^m)} + g(t_{k+1}^m,t_k^m)}_{\Upsilon(\tilde{x},T_k)}.
% \end{equation}
% We can similarly guarantee that $d_{\mathbb{X}_{t_{k}^m}}(\tilde{x}(t_{k}^m)) \leq 0$
% if 
% \begin{equation} \label{eq:tight_iter2}
% d_{\mathbb{X}_{t_{k+1}^m}}(\tilde{x}(t_{k+1}^m)) \leq \Upsilon(\tilde{x},T_k).
% \end{equation}
% In practice, the difference is that \eqref{eq:tight_iter} tightens constraints forwards in time, while \eqref{eq:tight_iter2} passes through the constraints backwards in time.

% The left and right hand sides of \eqref{eq:tight_iter} and \eqref{eq:tight_iter2} can be calculated from the approximate prediction $\tilde{x}(t)$. In Algorithm~\ref{alg:MR} we propose first iterating through a typical mesh-refinement procedure (lines \ref{line:MR1}--\ref{line:MR2}) to generate a prediction $\tilde{x}$ satisfying ODE error certificates in each segment.
% This sufficiently accurate prediction is then used as a proxy to evaluate \eqref{eq:tight_iter} on the refined mesh (lines \ref{line:t1}--\ref{line:t2}).

% The left and right hand sides of \eqref{eq:tight_iter} can be calculated form the approximate prediction $\tilde{x}(t)$. We propose iterating through a typical mesh-refinement procedure, (lines \ref{line:MR1}--\ref{line:MR2} in Algorithm~\ref{alg:MR}) to generate a prediction $\tilde{x}$ satisfying the ODE error certificates in each segment. This trajectory is then used as a proxy to evaluate \eqref{eq:tight_iter} at the refined mesh (lines \ref{line:t1}--\ref{line:t2} in Algorithm~\ref{alg:MR}).
% If \eqref{eq:tight_iter} is not satisfied at any time $t \in \mathcal{T}_k$ then the constraint set is tightened by
% \begin{equation}
%     \mathcal{B}_{\Upsilon_k} := \left\{x \in \mathbb{R}^n : \vecnorm{x} \leq \Upsilon(\tilde{x},T_k) \right\},    
% \end{equation}
% as in line~\ref{line:BallTight}, and the resulting NLP is resolved. Either the forward \eqref{eq:tight_iter} or backwards \eqref{eq:tight_iter2} may be used. 
% This procedure is repeated until \eqref{eq:tight_iter} is satisfied $\forall t \in T_h$.
% Intuitively, we are robustifying the problem formulation to inaccuracies in our solution method.
% This procedure is exemplified in Section~\ref{sec:NonlinearExample}.

% \begin{algorithm}
%     \caption{Adaptive Constraint Mesh Refinement Scheme}
%     \label{alg:MR}
%     \begin{algorithmic}[1] % The number tells where the line numbering should start
%         \Procedure{Mesh Refinement}{\ref{eq:Bolza_cont}, $\hat{\epsilon}$, $\mathcal{T}_h^0$, $J$}
%             \State $\epsilon_{k,i }\gets \infty, \ \forall k \in \mathcal{K}, i \in \{1,\hdots,n\}$ 
%             \State $j \gets 0$
%             \State $\mathbb{X}_s \gets \mathbb{X}\ominus\mathcal{B}_s$
%             \While{$\left( \exists \epsilon_{k,i} > \hat{\epsilon}_i\right)$} \label{line:MR1}
%                 \State $($\ref{eq:Bolza_cont}$_\text{NLP}^j)\gets$ Transcribe$(($\ref{eq:Bolza_cont}$_{\mathbb{X}_s}),\mathcal{T}_h^j)$ 
%                 \State $\tilde{x}(t),u(t) \gets \text{argmin }($\ref{eq:Bolza_cont}$_\text{NLP}^j)$
%                 \State Calculate $\epsilon_{k,i}, \ \forall k \in \mathcal{K}, i \in \{1,\hdots,n\}$
%                 \State $\mathcal{T}_h^{j+1} \gets \text{MeshRefinement} (\mathcal{T}_h^j,\epsilon)$
%                 \State $j \gets j+1$
%             \EndWhile \label{line:MR2}
%             \While{$\left(\exists t \in T_h : d_{\mathbb{X}_{t_{k}^m}}(\tilde{x}(t_{k}^m))\geq \Upsilon(\tilde{x}(\cdot),T_k)\right)$ } \label{line:t1}
%                 \State $\mathbb{X}_{t_k^m} \gets \mathbb{X}\ominus(\mathcal{B}_{t_k^m}\oplus\mathcal{B}_{\Upsilon_k})$ \label{line:BallTight}
%                 \State $($\ref{eq:Bolza_cont}$_\text{NLP}^j)\gets$ Transcribe$(($\ref{eq:Bolza_cont}$_{\mathbb{X}_{t_k^m}}),\mathcal{T}_h^j)$ 
%                 \State $\tilde{x}(t),u(t) \gets \text{argmin }($\ref{eq:Bolza_cont}$_\text{NLP}^j)$
%                 \State $j \gets j+1$
%             \EndWhile \label{line:t2}
%             \State \textbf{return} $\tilde{x}(t),u(t),\epsilon$
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

% \section{Example: Linear autonomous system} \label{sec:LinearExample}
% Consider the LTI autonomous system described by,
% \begin{equation} \label{eq:LinSys}
% \dot{x}(t) = Ax(t) + E\hat{w},
% \end{equation}
% \begin{equation} \label{eq:LinSysPar}
% x(t_0) = \begin{bmatrix} 10 \\ 10 \end{bmatrix}, \
% A = \begin{bmatrix}
% 0.05 & 0.5 \\
% 0 & -0.5
% \end{bmatrix}, \
% E = \begin{bmatrix}
% 1 \\
% 1
% \end{bmatrix},
% \end{equation}
% where $x \in \mathbb{R}^n$, simulated over $\Omega=6$\,s.
% We discretize $x(t)$ on a uniform coarse mesh with $h=1.5$\,s using either Forward Euler (FE),
% % where the approximate state $\tilde{x}(t)$ at mesh points $t_k \in \mathcal{T}_m =\{kh\}_{k\in\mathbb{R}^+}$ is,
% % \begin{equation}
% % \tilde{x}(t_{k+1}) = \tilde{x}(t_k) + A\tilde{x}(t_k), \  \tilde{x}(t_0)=x(t_0),
% % \end{equation}
% or a third-order Hermite-Simpson (HS) scheme.
% The FE discretization corresponds to a piece-wise linear trajectory reconstruction,
% % \begin{equation}
% % \tilde{x}(t) = \tilde{x}(t_k) + (t-t_k)\frac{x(t_{k+1})-x(t_k)}{h}, \ \forall t \in [t_k,t_{k+1}),
% % \end{equation}
% while the HS reconstruction is piece-wise cubic, and detailed in \cite{kelly2017introduction}.
% Fig.~\ref{fig:LinState} shows both approximations alongside the `true' and `nominal' trajectories $x(t),x^*(t)$ generated from Matlab's \texttt{linsim} function.
% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Figures/LinearStateTrajectories.eps}
% 	\caption[TODO]{A comparison of the true $x(t)$, the nominal $x^*(t)$ and the approximate $\tilde{x}(t) \in \mathcal{X}_{1}$ resulting from FE and HS collocation on a mesh with $h=1.5$, $\sigma=1$.}
% 	\label{fig:LinState}
% \end{figure}
% \begin{figure}[t!]
% 	\centering
% 	\vspace{0.5em}
% 	\subfloat[Approximation errors and quadratures. ]{
% 		\label{subfig:error1}
% 		\includegraphics[width=\columnwidth]{Figures/LinearErrors_1.eps}}

% 	\subfloat[Prediction errors of collocation schemes. ]{
% 		\label{subfig:error2}
% 		\includegraphics[width=\columnwidth]{Figures/LinearErrors_2.eps} }
% 	\caption{Plots of the approximation and prediction errors associated to the trajectories shown in Fig.~\ref{fig:LinState}.}
% 	\label{fig:LinErr}
% \end{figure}

% As seen in Fig.~\ref{subfig:error1}, the approximation error $\epsilon_i(t)$ and quadratures $\eta_{k,i}$ for the HS approximation are multiple orders of magnitude lower than the FE on the same mesh. For each scheme we posteriorly choose $\hat{\eta}= \max_k \eta_k$, which equals $3.8420$ in the case of FE and $0.0081$ for HS.
% As system \eqref{eq:LinSys} is unstable, the states in Fig.~\ref{fig:LinState} diverge and corresponding approximation errors grow.

% Corresponding to the different approximation errors, we chose an ETC threshold of $\hat{\epsilon}=5$ for the FE and $\hat{\epsilon}=0.5$ for the HS approximation. In both cases $\hat{\epsilon}>\hat{\eta}$ and the ETC condition \eqref{eq:EventTriggeringCondition} is met after $4.12$\,s and $1.7$\,s respectively. Fig.~\ref{subfig:error2} shows that the FE approximation error results in significant growth in $\epsilon(t)$. The minimum IUT $\underline{\tau}_u$ and times $\tau^\text{QET}, \tau^\text{CT}$ are detailed in Table~\ref{tab:1} for both approximations, and the associated functions plotted in Fig.~\ref{fig:LinTrig}.

% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Figures/LinearTriggeringTimes.eps}
% 	\caption[TODO]{A comparison of the online triggering estimations proposed in Section~\ref{sec:OnlineTrig} for FE and HS Schemes.}
% 	\label{fig:LinTrig}
% \end{figure}

% The line segments of $\text{QET-FE}(\eta)$ and $\text{QET-HS}(\eta)$ in Fig.~\ref{fig:LinTrig} have slope $L_x \hat{\epsilon} + \hat{w}$, and reflect state uncertainty due to $w(t)$. The discontinuities arise from the approximation errors. For FE scheme, $\underline{\tau}^u$ is significantly more conservative than $\tau^\text{QET}(\eta)$, whereas $\underline{\tau}^u \approx \tau^\text{QET}(\eta)$ for the HS. This is because $\underline{\tau}^u$ is estimated from the worst case absolute local error. From Fig.~\ref{fig:LinErr} the absolute difference between the errors in the first and last segment is orders of magnitude more than the difference between the errors in the first and last segment of the HS scheme.
% Using relative local error, as suggested in \cite[Ch. 5]{betts2010practical}, may result in better agreement between $\underline{\tau}$ and $\tau^\text{QET}(\eta)$ for the FE scheme.

% \begin{table}[ht]
% 	\centering
% 	\caption{Comparison of estimated IUTs.}
% 	\begin{tabular}{ l|c|c|c|c|c }
% 		& $\hat{\eta}$ & $\underline{\tau}^u$ & $\tau^\text{QET}(\eta)$ & $\tau^\text{QET}(\varepsilon)$ & $\tau^\text{CT}$ \\
% 		\hline\hline
% 		FE $(\hat\epsilon=5)$ & $0.1$ & $0.25$ & $1.49$ & $1.74$ & $1.39$ \\
% 		HS $(\hat\epsilon=0.5)$ & $ 0.045$ & $1.22$  & $ 1.27$ & $1.28$ & $0.4$ \\
% 	\end{tabular} \label{tab:1}
% \end{table}

% \section{Closed Loop Simulation} \label{sec:NonlinearExample}

% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Images/TwoLinkRobotArmPlant}
% 	\caption[TODO]{The two link robot arm plant considered in closed loop simulations}
% 	\label{fig:TwoLinkRobotArm}
% \end{figure}
% We now consider a closed-loop example of the two link robotic arm, shown in Figure~\ref{fig:TwoLinkRobotArm}, over a simulation time of $8$\,s. 
% We employ the quadratic objective function
% \begin{equation}
% \int_{t_0}^{t_f} u_1^2(t) + u_2^2(t) \mathrm{d}t,
% \end{equation}
% which is often interpreted as a minimum energy objective, over a receding horizon of length $T_\text{OP}=4$\,s. The input input $u\in\mathbb{R}^2$, and the state is characterised as $x:=[\omega_\alpha, \   \omega_\beta, \ \theta, \ \beta]$. $\omega_\alpha$ and $\omega_\beta$ are the angular accelerations of each joint in the arm and $\theta, \ \beta$ the corresponding angular velocities. The nonlinear time-invariant dynamics $f(x,u)$ are described by
% \begin{align}
%     \dot\omega_\alpha(t) &= \Big(\frac{9}{4}\sin(\theta(t))\cos(\theta(t))x_1(t)^2 + 2x_2(t)^2 +
%     \frac{4}{3}u_1(t) - \\ & \quad \quad \frac{4}{3}u_2(t) - \frac{3}{2}\cos(\theta(t))u_2(t)\Big)
%     \Big(\frac{31}{36} + \frac{9}{4}\sin^2(\theta(t))\Big)^{-1}, \\
%     \dot\omega_\alpha(t) &= \Big(\frac{9}{4}\sin(\theta(t))\cos(\theta(t))x_2(t)^2 + \frac{7}{2}x_1(t)^2 - \frac{7}{3}u_2(t) + \\ & \frac{3}{2}\cos(\theta(t))\left(u_1(t)-u_2(t)\right)\Big) \Big(\frac{31}{36} + \frac{9}{4}\sin^2(\theta(t))\Big)^{-1}, \\
%     \dot\theta(t) &= \omega_\alpha(t) - \omega_\beta(t), \\
%     \dot\beta(t) &= \omega_\beta(t).
%     \label{eq:floatingeq}
% \end{align}
% Each state is additionally effected with additive noise $v(t) \in \mathbb{R}^4, \vecnorm{v(t)}\leq 5\times 10^3$.
% Using the method described in \cite{khalil2002nonlinear}, we estimate the Lipschitz constant of the system as $L_x=4.5309$.
% We employ a trapezoidal collocation, detailed in \cite{kelly2017introduction}, where linear input and quadratic state reconstruction is assumed. 

% We base the mesh refinement steps in Algorithm~\ref{alg:MR} on the algorithm in \cite[Ch.5]{betts2010practical}, with refinemtn based on condition \eqref{eq:AbsoluteLocalError} with $\hat{\epsilon}_i=10^{-3}$. The refinement phase of Algorithm~\ref{alg:MR} terminates when \eqref{eq:AbsoluteLocalError} in each mesh segment, after which we perform constraint tightening.
% We constrain the angular acceleration of the first joint to be $\omega_\alpha\in[-0.3,0.3]$. A viable distance operator may be used with the presence of additional constraints through the method proposed in \cite{fontes2018guaranteed}.

% We consider two different closed loop update scenarios. In scenario a) the ETC scheme is used to trigger control updates based on the one-norm of the difference between predicted state $\tilde{x}(t)$ and measured state $x(t)$ using condition \eqref{eq:EventTriggeringCondition} with threshold $\Delta=7\times10^{-3}$. 
% In scheme b) we pose a self-triggered control setup, where updates are performed at times in accordance with Theorem~\ref{th:QET}, also with threshold $\Delta=7\times10^{-3}$. 
% The closed-loop state and input trajectories are shown in Figures~\ref{fig:NL_State} and \ref{fig:NL_Input}. The subscripts $E$ and $S$ are respectively used to denote the closed-loop trajectory for the event- and self-triggered update schemes. 

% The crosses in Figure~\ref{fig:NL_State} are used to show the location of the mesh points of the concatenated closed-loop solution. The update times $\mathcal{T}_u$ for the ETC and STC scenarios are shown by the black and blue open circles. Notably the IUTs of the ETC scheme are significantly less significant than the STC IUTs, with updates on average every $2.69$\,s. Conversely, condition \eqref{eq:trig_QET} results in updates on average every $0.48$\,s. 
% The closed-loop cost of the ETC scheme is $0.1335$, while the increased triggering of the STC scheme costs $0.1243$.
% However, it is important to note that \eqref{eq:trig_QET} does not use any knowledge of the predicted or measured state -- but only on the error in the solution of the OCP guaranteed by the mesh refinement algorithm. Even just triggering on condition \eqref{eq:trig_QET}, the IUTs do increase as the reaches the terminal condition. Future work should consider a condition which depends on both the predicted state $\tilde{x}$ \emph{and} the quadrature errors $\epsilon_k$.

% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Figures/CL_RobotArm_Input.eps}
% 	\caption[TODO]{Closed loop input trajectories and control update times for the ETC scheme and STC scheme based on Theorem~\ref{th:QET}.}
% 	\label{fig:NL_Input}
% \end{figure}

% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Figures/CL_RobotArm_State.eps}
% 	\caption[TODO]{Closed loop state trajectories and control update times for the ETC scheme and STC scheme based on Theorem~\ref{th:QET}. The crosses depict the combined NLP solution of the ETC solves.}
% 	\label{fig:NL_State}
% \end{figure}

% The proposed triggering does account for proximity to constraints. Using Theorem~\ref{th:tight} we can guarantee constraint satisfaction of the continuous time plant in both the event- and self-triggered schemes. At each update we apply the two stage tightening procedure in Algorithm~\ref{alg:MR}. The result of the first solve at time $t=0$ is shown in Figure~\ref{fig:NL_ConstTight} for the constrained state $\omega_\alpha(t)$. The dashed red line shows the first stage of the procedure, where constrain tightening is based on $\mathcal{B}_s$. The black line shows the predicted state trajectory using only this first stage of tightening. As shown, the quadratic sate interpolation results in the predicted state violating the tightened constraint. In this case we cannot guarantee constraint satisfaction of the real plant at these times. 
% The second stage of tightening, at discrete times $\mathcal{T}_m$, is shown by the blue dots. For clarity of representation, we mimic the tightening of the upper and lower bounds. Nominally, for a sufficiently dense mesh the trajectory of the tightened problem and non-tightened problem are similar. 

% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Figures/OL_RobotArm_Constraint.eps}
% 	\caption[TODO]{An example of the constraint tightening mesh-refinement procedure proposed in Section~\ref{sec:constraintTightening} and Algorithm~\ref{alg:MR}. The black line shows the state refined state trajectory after the constraint set is tightened from $\mathbb{X}$ to $\mathbb{X}_s$. The pink link shows the final trajectory after the constraints are additionally iteratively tightened.The blue dots show the final constraint bounds at the mesh points.}
% 	\label{fig:NL_ConstTight}
% \end{figure}

% Finally, in Figure~\ref{fig:CompComparison} we consider how different combinations of thresholds $(\Delta,\hat\epsilon)$ result in both a different computational load, and a different distribution of computation in time for the ETC scheme. As the threshold $\Delta$ increases, the number of control updates and the time spent in IPOPT decreases. We also see that as the quality of the prediction improves, the number of updates decreases (up to a point), but the total time in IPOPT tends to increase. 


% \begin{figure}[tb]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Figures/ComputationTimeComparison.eps}
% 	\caption[TODO]{Comparison of computation time and number of control updates for various ETC and refinement conditions $(\hat{\epsilon},\Delta)$}
% 	\label{fig:CompComparison}
% \end{figure}


